Deep density networks and uncertainty in recommender systems

Building robust online content recommendation systems requires learning complex interactions between user preferences and content features. The field has evolved rapidly in recent years from traditional multi-arm bandit and collaborative filtering techniques, with new methods employing Deep Learning models to capture non-linearities. Despite progress, the dynamic nature of online recommendations still poses great challenges, such as finding the delicate balance between exploration and exploitation. In this paper we show how uncertainty estimations can be incorporated by employing them in an optimistic exploitation/exploration strategy for more efficient exploration of new recommendations. We provide a novel hybrid deep neural network model, Deep Density Networks (DDN), which integrates content-based deep learning models with a collaborative scheme that is able to robustly model and estimate uncertainty. Finally, we present online and offline results after incorporating DNN into a real world content recommendation system that serves billions of recommendations per day, and show the benefit of using DDN in practice.

==> abstract.tex <==
Building robust online content recommendation systems requires learning complex interactions between user preferences and content features. The field has evolved rapidly in recent years from traditional multi-arm bandit and collaborative filtering techniques, with new methods integrating Deep Learning models that enable to capture non-linear feature interactions. Despite progress, the dynamic nature of online recommendations still poses great challenges, such as finding the delicate balance between exploration and exploitation.  In this paper we provide a novel method, Deep Density Networks (DDN) which deconvolves measurement and data uncertainties and predicts probability density of CTR (Click Through Rate), enabling us to perform more efficient exploration of the feature space. We show the usefulness of using DDN online in a real world content recommendation system that serves billions of recommendations per day, and present online and offline results to evaluate the benefit of using DDN.







==> literature.tex <==
% Deep learning & Recomendation systems
%Over the past decade deep learning has been applied with tremendous success in many different application domains such as computer vision, speech recognition and machine translation.  In recent years we have seen a corresponding explosion of deep learning models in the recommender systems landscape, revolutionizing recommendation architectures and providing superior performance over traditional models \cite{zhang2017deep,cheng2016wide, covington2016deep, okura2017embedding}. Deep learning's ability to capture non-linearities has enabled to model complex user-item relations and to integrate higher level representations of data sources such as contextual, textual and visual input.

Traditionally, algorithmic modelling in recommendation systems can be classified into either Collaborative Filtering (CF) or content-based methods. CF methods use past user-item interactions to predict future ratings~\cite{linden2003amazon}. The most popular approach for CF is Matrix Factorization (MF), where items and users are represented in a common latent space and ratings are computed as the inner product between the user and item representations~\cite{mnih2008probabilistic}. A drawback to MF approaches is the so called item cold-start (ICS) problem, i.e. they fail to apply to new users/items. In order to handle ICS, content-based approaches use meta-information about the new items. %, but are missing the interaction between users. 
The contrast between these two methods can be seen as a trade-off between memorization of users/items seen in the past, compared to generalization for new items. Hybrid methods that combine both the memorization advantages of MF with the generalization achieved by content-based methods have been proposed ~\ref{cheng2016wide}. We use this hybrid approach, by employing deep neural networks to learn item representations and combine those with contextual features. 

In order to improve the performance of prediction quality and tackle faster the ICS problem, recommender systems have been modeled in a multi-arm bandit setting, where the goal is to find an exploitation/exploration selection strategy that maximizes the long term reward~\cite{li2010contextual}.
%
A similar challenge has been faced in Reinforcement learning (RL) setting, in which an agent has to decide when to forego an immediate reward and to explore its environment. 
%
Bayesian neural networks (\cite{neal2012bayesian}) using distributions over the weights were applied by using either sampling or stochastic variational inference (\cite{kingma2013auto, rezende2014stochastic}). 
%While Bayesian models offer a mathematically grounded framework, they usually entail a prohibitive computational cost. 
%
\cite{blundell2015weight} proposed Bayes by Backprop algorithm for the variational posterior estimation and applied Thompson sampling in multi-arm bandit setting similarly to our case. 
\cite{gal2016dropout} proposed Monte Carlo (MC) dropout, a Bayesian approximation of model uncertainty by extracting estimations from the different sub-models that have been trained using dropout.  
% MDN & classification
Building upon their previous work the authors separated uncertainty into two types, model and data uncertainty, while studying the effect of each uncertainty separately in computer vision tasks~\cite{kendall2017uncertainties}. 
%
Similarly, we separate recommendation prediction uncertainty into three types: measurement, data and model uncertainty.  
In addition, in contrast to~\cite{zhu2017deep} where homoscedastic data uncertainty was assumed, we assumed heteroscedastic data uncertainty which is a more natural choice for recommendation systems.  
%
%
%Mixture density networks (MDN) (\cite{bishop1994mixture}) were shown to have the ability to model data uncertainty directly. 
%
Our work also has parallels to \cite{li2010contextual} where the authors formulated the exploration/exploitation trade-off in personalized article recommendation as a contextual bandit problem and proposed LinUCB algorithm, which adapts the UCB strategy to support models based on contextual features. Our approach extends LinUCB by using a deep model and incorporating diverse types of uncertainty. 
%
%Furthermore, recently \cite{zhu2017deep} also proposed a deep model with model and data uncertainty estimations for time series prediction, however they assumed homoscedastic data uncertainty in contrast to our case where we assumed heteroscedastic data uncertainty and so our estimations were dependent on the specific input. 

%In contrast to LinUCB, we use a deep network architechture, 

%The difference to our approach is that we are employing a hybrid deep neural network model for explicitly modeling the content-based information about the items and uncertainty estimation. 
%We are employing MDN to estimate data uncertainty and exploit this information for more efficient exploration of the feature space. 

The effect of measurement noise and noisy labels has been studied extensively (\cite{frenay2014classification}). 
\cite{mnih2012learning} proposed a probabilistic model for the conditional probability of seeing a wrong label, where the correct label is a latent variable of the model. 
\cite{goldberger2016training} explicitly modeled noise by an additional softmax layer that connects the correct labels to the noisy ones. 
%
Inspired by these works, in this paper we model measurement noise using a Gaussian model and combine it with Gaussian Mixture Model (GMM) to form a deep Mixture density network (MDN)\cite{bishop1994mixture}. 
